Integration of Quantum Accelerators with High Performance Computing -- A Review of Quantum Programming Tools

Quantum computing (QC) introduces a novel mode of computation with the possibility of greater computational power that remains to be exploited - presenting exciting opportunities for high performance computing (HPC) applications. However, recent advancements in the field have made clear that QC does not supplant conventional HPC, but can rather be incorporated into current heterogeneous HPC infrastructures as an additional accelerator, thereby enabling the optimal utilization of both paradigms. The desire for such integration significantly affects the development of software for quantum computers, which in turn influences the necessary software infrastructure. To date, previous review papers have investigated various quantum programming tools (QPTs) (such as languages, libraries, frameworks) in their ability to program, compile, and execute quantum circuits. However, the integration effort with classical HPC frameworks or systems has not been addressed. This study aims to characterize existing QPTs from an HPC perspective, investigating if existing QPTs have the potential to be efficiently integrated with classical computing models and determining where work is still required. This work structures a set of criteria into an analysis blueprint that enables HPC scientists to assess whether a QPT is suitable for the quantum-accelerated classical application at hand.

==> glossary.tex <==
\section{Glossary}
\MG{Since we now have a live glossary, I'd restrict this table to the terms used in the paper. After all, every definition here might be outdated soon}
\AMR{Let's wait and see whether it is best to include it all as a contribution toward a unified definition in the community or not}
\MG{I would remove the glossary. It's not strictly necessary for this paper and since the website has already been criticized, the same will probably also happen for this table, if we don't justify or cite each and every term's definition.}

The glossary provides an overview over commonly used terms in the quantum computing context.
\MG{Quantum computing and quantum compilation context maybe?}
\AMR{Given the fact that Physicists were not that happy with the glossary, would it make sense to add for each expression both the "computer scientist perspective" and the "physicists perspective"? We can ask the PIs to give their input regarding this.}
As many different disciplines are entailed, the glossary provides the definitions as used by us which is in no means absolute. A more extensive live document can be found at \url{https://quantum-glossary.github.io/}.
\newcommand*{\nope}{{\color{red}\textbf{X}}} %
\begin{longtable}{>{\raggedright}p{3cm}@{\hspace{0.5cm}}p{8.5cm}}\toprule
    \textbf{Expression} & \textbf{Definition} \\* \midrule\endhead
    Circuit Execution Time & The quantum equivalent of the runtime, the duration a quantum circuit runs from start to full measurement. Usually accounts for the fact that quantum circuits have to be executed a certain number of times (called shots). Parameters may be filled in during this step. For hybrid programs, this is included in the runtime. \newline \emph{Synonyms} Quantum Runtime \newline \emph{Related Terms} Runtime, Coherence time \\* \midrule 
    Circuit Generation Time & The point in time from when a quantum circuit is constructed (including all necessary pre-calculations) until it is fully defined. Usually, it is followed by or includes optimization steps. In parametrized circuits, parameters don't have to be filled in yet! \newline \emph{Related Terms} Parametrized Circuit \\* \midrule 
    Classical Compilation Time & "The runtime of the Compiler" before the runtime of the program. Optimizations during the compilation time are called offline. \\* \midrule 
    Coherence Time & Figuratively, the time it takes for a quantum state to be subject to energy decay or dephasing, limiting the operation fidelity on the qudits involved. The $T_1$-time (spin-lattice/longitudinal relaxation time) describes the probability of a qubit still being in $\ket{1}$ after time $t$. The $T_2$-time (spin-spin/transverse relaxation time) describes the probability of a qubit still being in $\ket{+}$ after time $t$.
 \newline \emph{Synonyms} Lifetime \\* \midrule 
    Compilation & General term for the processing of abstract description into an actualized, generally more detailed representation. The general steps in classical compilation include Lexing, Parsing and Transformation. During the transformation step, usually some optimization techniques are applied. Compilation is also often used to describe the processing of a program written in an abstract programming language, into an executable binary. There are two major approaches for compilation, namely Ahead-of-time (AOT) and Just-in-time (JIT). \newline \emph{Related Terms} Optimization, Compilation Toolchain, Performance Aware Compilation \\* \midrule 
    Compilation Toolchain & Compilation processes have grown more complex over time. A compilation toolchain usually describes all necessary tools to go from the highest level of abstraction to the lowest level. In some instances it covers only a selection of chained tools. It includes the flow of data through the different tools, optimization techniques at various intermediate levels and interface descriptions to plug in new tools.\\* \midrule 
    Domain Specific Language & A Domain Specific Language (DSL) is tailored to a fixed domain. They serve a specialized purpose and are usually not complete. Instead, they extend existing languages. \\* \midrule 
    Dynamic Lifting & Originally termed by quipper~\cite{green2013quipper} as the conversion from measurement results (bit) to classical value (bool). During dynamic lifting, the quantum operations are suspended to execute classical operations, which govern the future circuit execution. The classical execution has to complete during the coherence time and therefore requires execution on the controller as sending information over a bus would be intractable.\newline \emph{Synonyms} Real-Time Feedback \newline \emph{Related Terms} Coherence Time \\* \midrule 
    Execution Model & The model which governs the execution of a program. The execution model defines the behavior between different components in the programming language, the interaction between the classical computer and the quantum computer (intermediate or non-intermediate) including scheduling. The execution model is enforced by the runtime environment. The program execution can be defined by operational semantics. In quantum computing three models have been defined~\cite{fu2021quingo}; The \gls{QRAM} Model, the Restricted \gls{HQCC} Model and the Refined \gls{HQCC} Model. \newline \emph{Related Terms} Runtime Environment \\* \midrule 
    Framework & A framework redefines and controls the execution model of a programming language. This might change the way how to write a typical program. Frameworks provide a fixed purpose and functionality. \\* \midrule 
    Library & A library provides a fixed functionality to its host programming language. It defines a clear interface for interaction with the functionality. \\* \midrule 
    Mapping & The association of logical qudits used in an abstract quantum algorithm to physical qudits in a quantum system, under constraints of the physical coupling. In quantum computing this is the relation of abstract signal lines to physical signal lines connected to a qudit. \newline \emph{Related Terms} Coupling Graph \\* \midrule
    Native gate set & The set of unitary operations that are physically available on a given chip. Usually provide a fidelity measure for each operation. \newline \emph{Synonyms} Atomic gate set, Basic or Basis gate set, Elementary gates \newline \emph{Related Terms} Universal Gate Set, Fidelity \\* \midrule 
    Near-Time feedback & Communication within a hybrid node, between classical and quantum components. Communication can freely occur between shots. \newline \emph{Related Terms} Quantum Enable Node \\* \midrule 
    Parametrized Circuit & A parametrized circuit consists of a set of parametrized and fixed gates. The overall structure of the circuit doesn't change, only the parameters are updated. They are often used in variational algorithms. \\* \midrule 
    Platform & The type of physical system used to implement quantum computations. The most common types are ion traps, superconduction qubits, photonic quantum computers, quantum annealers and Rydberg atoms. \\* \midrule
    Programming Language & A programming language is a set of tools to define a program. Programming languages are defined by formal semantic rules and have at least a properly defined grammar. \newline \emph{Synonyms} General Purpose Language (GPL), Language \\* \midrule 
    Programming Model & A model for writing programs to facilitate a specific execution model. This might be different from the intended execution model of the underlying language. This is usually implemented in or enforced by a framework. A common example for parallel computing is MapReduce~\cite{dean2010system}. \newline \emph{Related Terms} Framework \\* \midrule
    Quantum Compilation Time & "The runtime of the Quantum Compiler". It can occur during the runtime (during Circuit Generation Time) \textbf{OR} compilation time of the classical program. \\* \midrule   
    Quantum Enabled Node & Full stack for quantum-classical hybrid operations including classical hardware, quantum hardware and communication hardware. \newline \emph{Synonyms} Machine, Device \\* \midrule 
    Quantum Hardware & All hardware necessary to operate a specific quantum platform. Some components included are waveform generators, digital-analog and analog-digital converters, and a microcontroller or FPGA. \\* \midrule 
    Quantum Operations & All possible operations that can be executed on qudits. The operations can be grouped in two sets. Reversible, unitary operations called gates and irreversible, non-unitary operations. \newline \emph{Related Terms} Qudits \\* \midrule 
    Routing & The process that ensures (decomposed) gates in a circuit satisfy the coupling constraints, for example nearest-neighbor interactions. This is done using SWAP gates and BRIDGE gates.\\* \midrule 
    Runtime & The runtime is the time a program runs from its start until its termination. Optimizations during the runtime are called online.\newline \emph{Synonyms} (Classical) Execution Time \\* \midrule 
    Runtime Environment & The runtime environment (commonly referred to as runtime) is the underlying system for executing a program. It includes resource management, especially memory allocation and garbage collection Supporting libraries or frameworks for example message passing,  and interfaces to hardware. For performance reasons, some of these tasks are relegated to the operating system. \textbf{Interpretation} of code is usually understood as part of the runtime, while \textbf{Compilation is not}. Compilers are tightly integrated into the runtime environment but technically not part of it.  \newline \emph{Synonyms} Runtime \\* \midrule 
    Scheduling & Scheduling refers to the task of distributing restricted resources (CPU, QPU,...) between different parties (processes, users). The execution queue of jobs is called a \textbf{schedule}. Scheduling can occur on different levels. On a job level user access to computing resources are managed. On a process level, shared resources between processes are managed. In quantum computing, scheduling can be applied on a circuit level, ordering the application of gates. Scheduling is usually handled by the runtime environment. \newline \emph{Related Terms} Runtime Environment \\* \midrule
    Transpilation & General term for the processing of abstract description into a representation on the same level of abstraction. In quantum computing, during transpilation the circuit representation is translated to another circuit representation under different constraints and can include circuit optimization. Common examples are decomposition of all gates to the native gate set of a given hardware and gate cancellation. Transpilation is \textbf{wrongly} used synonymously to compilation. Instead, transpilation is a specific type of compilation. It is sometimes used to refer to individual steps during compilation. The use of the term \textbf{transpilation} is also highly controversial.\\* %
    \bottomrule 

\end{longtable}
